Parallel Approximate Undirected Shortest Paths Via Low Hop Emulators

We present a $(1+\varepsilon)$-approximate parallel algorithm for computing shortest paths in undirected graphs, achieving $\mathrm{poly}(\log n)$ depth and $m\mathrm{poly}(\log n)$ work for $n$-nodes $m$-edges graphs. Although sequential algorithms with (nearly) optimal running time have been known for several decades, near-optimal parallel algorithms have turned out to be a much tougher challenge. For $(1+\varepsilon)$-approximation, all prior algorithms with $\mathrm{poly}(\log n)$ depth perform at least $\Omega(mn^{c})$ work for some constant $c>0$. Improving this long-standing upper bound obtained by Cohen (STOC'94) has been open for $25$ years. We develop several new tools of independent interest. One of them is a new notion beyond hopsets --- low hop emulator --- a $\mathrm{poly}(\log n)$-approximate emulator graph in which every shortest path has at most $O(\log\log n)$ hops (edges). Direct applications of the low hop emulators are parallel algorithms for $\mathrm{poly}(\log n)$-approximate single source shortest path (SSSP), Bourgain's embedding, metric tree embedding, and low diameter decomposition, all with $\mathrm{poly}(\log n)$ depth and $m\mathrm{poly}(\log n)$ work. To boost the approximation ratio to $(1+\varepsilon)$, we introduce compressible preconditioners and apply it inside Sherman's framework (SODA'17) to solve the more general problem of uncapacitated minimum cost flow (a.k.a., transshipment problem). Our algorithm computes a $(1+\varepsilon)$-approximate uncapacitated minimum cost flow in $\mathrm{poly}(\log n)$ depth using $m\mathrm{poly}(\log n)$ work. As a consequence, it also improves the state-of-the-art sequential running time from $m\cdot 2^{O(\sqrt{\log n})}$ to $m\mathrm{poly}(\log n)$.

==> ourResults.tex <==
\subsection{Our Results}

We now further discuss our results on parallel computation of the $(1+\varepsilon)$-approximate shortest path.
Some of our results have new consequences beyond parallel algorithms:
including faster sequential algorithms and constructions where none
were previously known. 
Our input is a connected $n$-vertex $m$-edge undirected weighted graph $G=(V,E,w)$ with weights $w:E\rightarrow \mathbb{Z}_{\geq 0}$ and $\max_{e\in E}w(e)\leq \poly(n)$.
The parallel algorithms from this paper are in the EREW PRAM model.

\paragraph{Low hop emulator and applications.} 
\csnote{Do we need this first paragraph?  We already defined low hop emulator above}
An emulator of $G$ is a sparse graph $G'=(V,E',w')$ such that for any two vertices $u,v\in V$, $\dist_{G'}(u,v)$ is a good approximation to $\dist_G(u,v)$.
We extend the definition of emulator to further require $G'$ to have a low hop diameter (see Section~\ref{sec:preli} for more details), i.e., for any two vertices $u,v$ in $G'$, there exists a shortest path between $u,v$ which only uses small number of edges (hops).

We give an efficient parallel sparse low hop emulator construction
algorithm.  To the best of our knowledge, it was not even clear
whether a sparse low hop emulators exist, and thus no previous
algorithm was known even in the sequential setting.

\begin{theorem}[Low hop emulator, restatement of Theorem~\ref{thm:parallel_low_hop_emulator}]
  For any $k\geq 1$, any graph $G$ admits a low hop emulator
  $G'$, with expected size of $\wt{O}\left(n^{1+\frac{1}{k}}\right)$,\footnote{$\wt{O}(f(n))$ denotes $f(n)\cdot \poly\log(f(n))$.} satisfying:
\begin{align*}
\forall u,v\in V, \dist_{G}(u,v)\leq \dist_{G'}(u,v)\leq \poly(k)\cdot \dist_G(u,v),
\end{align*}
and with the hop diameter at most $O(\log k)$.
Furthermore, there is a PRAM algorithm computing the emulator $G'$ in
  $\poly\log(n)$ parallel time using $\wt{O}(m+n^{1+\frac{2}{k}})$ expected work.
\end{theorem}

Notice that in the case of $k=\log n$, we can compute a low hop emulator with expected size $\wt{O}(n)$ and hop diameter $O(\log\log n)$ in $\poly\log(n)$ parallel time using $\wt{O}(m)$ expected work.
The approximation ratio in this case is $\poly\log(n)$.

There are many applications of low hop emulators for parallel graph
algorithm design.
We list a few of them here.
In all of these applications, the depth is $\poly\log(n)$ and the expected work is $\wt{O}(m)$.
The first direct application is a parallel algorithm for $\poly(\log n)$-approximate single source shortest path (SSSP).
By applying Bellman-Ford algorithm on the low hop emulator, we can compute a $\poly(\log n)$-approximate distance from a source vertex $s$ to every other vertex $v$ (see Corollary~\ref{cor:parallel_sssp}). 
The second application is a parallel version of Bourgain's embedding~\cite{b85}.
We can efficiently embed a graph metric into a $\poly\log n$ dimensional $\ell_1$ space in parallel (see Corollary~\ref{cor:parallel_embed_into_l1}).
This embedding algorithm is also a crucial building block in our parallel uncapacitated minimum cost flow algorithm and $s-t$ shortest path algorithm.
\begin{comment}
\begin{corollary}[Parallel Bourgain's embedding, restatement of Corollary~\ref{cor:parallel_embed_into_l1}]\label{cor:parallel_embed_into_l1_informal}
Given a graph $G=(V,E,w)$, there is a PRAM algorithm which outputs a mapping $\varphi:V\rightarrow \ell_1^d$ for $d=O(\log^2 n)$ in $\poly\log(n)$ parallel time using $\wt{O}(m)$ expected work such that with probability at least $0.99$,
\begin{align*}
\forall u,v\in V, \dist_{G}(u,v)\leq \|\varphi(u)-\varphi(v)\|_1 \leq \poly\log(n)\cdot \dist_G(u,v).
\end{align*}
\end{corollary}
\end{comment}
The third application is a parallel metric tree embedding algorithm.
By applying parallel FRT embedding~\cite{frt04,fl18} on the $\wt{O}(n)$ size low hop emulator, we can improve the efficiency of the parallel metric tree embedding algorithm (see Corollary~\ref{cor:parallel_metric_tree}).
\begin{comment}
\begin{corollary}[Parallel metric tree embedding, restatement of Corollary~\ref{cor:parallel_metric_tree}]
Given a graph $G=(V,E,w)$, there is a PRAM algorithm which outputs a tree $T=(V',E',w')$ in $\poly\log(n)$ parallel time using $\wt{O}(m)$ expected work such that $\forall u,v\in V$, 
\begin{align*}
\begin{array}{ccc}
\dist_G(u,v)\leq \dist_T(u,v) &\text{~and~}& \E_T[\dist_T(u,v)]\leq \poly\log(n)\cdot \dist_G(u,v).
\end{array}
\end{align*}
\end{corollary} 
\end{comment}
The forth application is parallel low diameter decomposition.
By applying parallel low diameter decomposition algorithm~\cite{mpx13} on the $\wt{O}(n)$ size low hop emulator, we can get a more efficient parallel low diameter decomposition algorithm (see Corollary~\ref{cor:parallel_ldd}). %the following parallel low diameter decomposition result.
\begin{comment}
\begin{corollary}[Parallel low diameter decomposition, restatement of Corollary~\ref{cor:parallel_ldd}]
Given a graph $G=(V,E,w)$ and a parameter $\beta\in(0,1]$, there is a PRAM algorithm which partitions $V$ into subsets $C_1,C_2,\cdots, C_k$ in $\poly\log(n)$ parallel time using $\wt{O}(m)$ expected work such that 
\begin{enumerate}
\item $\forall i\in[k],~\forall u,v\in C_i,~\dist_G(u,v)\leq \frac{\poly\log(n)}{\beta}$,
\item $\forall u,v\in V,~\Pr[u,v\text{ are not in the same subset}]\leq \beta\cdot \dist_G(u,v)$.
\end{enumerate}
\end{corollary}
\end{comment}

%An another byproduct of our low hop emulator algorithm is a work efficient $\wt{O}(n)$ size distance oracle algorithm. 
%A distance oracle is a static data structure which uses small space and can be used to efficiently return an approximate distance of any pair of query vertices.

%\begin{theorem}[$\wt{O}(n)$ size distance oracle, a modified version of Theorem~\ref{thm:parallel_dis_oracle}]
%There is a PRAM algorithm which preprocesses an input graph $G$ in $\poly\log(n)$ parallel time using $\wt{O}(m)$ work and outputs a size $\wt{O}(n)$ data structure such that for any pair of vertices $u,v$, a $\poly\log(n)$ approximate distance can be computed in $O(\log\log n)$ time given the data structure.
%\end{theorem}

\paragraph{Uncapacitated minimum cost flow and Approximate $s-t$ shortest path.}
In the uncapacitated minimum cost flow problem, also known as the
transshipment problem, given a demand vector $b\in\mathbb{R}^n$ satisfying $\sum_{v\in V} b_v = 0$,
the goal is to determine the flow on each edge such that the demand of
each vertex is satisfied and the cost of the flow is minimized. Formally, we want to solve
\begin{align*}
&\min_{f} \sum_{e:~e=\{u,v\}\in E} |f(u,v)| \cdot w(e)\\
\text{s.t.~}&\forall u\in V,\sum_{v:\{u,v\}\in E} f(u,v) = b_u,\\
&\forall u,v\in V, f(u,v)=-f(v,u).
\end{align*}
Based on our parallel Bourgain's embedding (Corollary~\ref{cor:parallel_embed_into_l1}), we give a novel construction of the preconditioner for uncapacitated minimum cost flow problem.
By plugging the new preconditioner into Sherman's framework~\cite{s17}, we give a parallel algorithm which computes a $(1+\varepsilon)$-approximate uncapacitated minimum cost flow in $\poly\log(n)$ parallel time using $\wt{O}(m)$ work.
\begin{theorem}[Parallel uncapacitated minimum cost flow, restatement of Theorem~\ref{thm:parallel_min_cost_flow}]
	Given a graph $G=(V,E,w)$, a demand vector $b\in\mathbb{R}^{n}$ and an error parameter $\varepsilon\in(0,0.5)$, there is a PRAM algorithm which outputs an $(1+\varepsilon)$-approximate solution to the uncapacitated minimum cost flow problem with probability at least $0.99$ in $\varepsilon^{-2}\poly\log(n)$ parallel time using $\wt{O}(\varepsilon^{-2}m)$ expected work.
\end{theorem}
Notice that our parallel algorithm also implies that computing a $(1+\varepsilon)$-approximate solution to the uncapcitated minimum cost flow problem can be done in $\wt{O}(\varepsilon^{-2}m)$ time in the sequential setting.

This algorithm suffices for estimating the shortest path distance
$\dist_G(s,t)$ for any two vertices $s,t\in V$: if we set the demand
vector as $b_s=1,b_t=-1$ and $b_u=0$ for $u\not=s,t$, then the optimal
cost of uncapacitated minimum cost flow problem yields the answer.
However, this is not enough for computing a corresponding approximate
shortest path: our flow algorithm outputs an approximate shortest path
flow, which may be non-integral and cyclic.

Hence we develop a further algorithm which actually constructs a path
connecting $s$ and $t$, using parallel recursive path construction,
described in the next section.

\begin{theorem}[Parallel $(1+\varepsilon)$-approximate $s-t$ shortest path, restatement of Theorem~\ref{thm:st_shortest_path}]
Given a graph $G=(V,E,w)$, two vertices $s,t\in V$ and an error parameter $\varepsilon\in (0,0.5)$, there is a PRAM algorithm which can output a $(1+\varepsilon)$-approximate $s-t$ shortest path with probability at least $0.99$ in $\varepsilon^{-2}\poly\log(n)$ parallel time using expected $\wt{O}(\varepsilon^{-3}m)$ work.
\end{theorem}

